Ambient and high pressure studies of structural, electronic and magnetic properties of EuZn$_2$P$_2$ single crystal

A thorough study of EuZn$_2$P$_2$ single crystals, which were grown from Sn flux, was performed using both bulk (heat capacity, ac susceptibility, dc magnetization, electrical resistivitivity, magnetoresistance) and microscopic (M\"ossbauer spectroscopy) techniques. Electrical resistance and magnetic susceptibility were measured also under high pressure conditions (up to 19 GPa and 9.5 GPa, respectively). Further insight into electronic properties and phonons is provided by ab initio calculations. The results indicate that EuZn$_2$P$_2$ is an antiferromagnet with strong Eu-Eu exchange coupling of ferromagnetic type within the basal plane and weaker antiferromagnetic interaction along the c axis. The Eu magnetic moments are tilted from the basal plane. Hydrostatic pressure strongly affects both magnetic (increase of the N\'eel temperature) and electronic (suppression of the band gap and semi metallic behavior) properties, indicating a strong interplay of structure with magnetic and electronic degrees of freedom.

==> a_Abstrakt.tex <==
%Jakie były pomiary zrobione
%Magnetyczny Diagram fazowy
%Pomiary pod ciśnieniem
%Badanie stanu podstawowego/typu uporządkowania
%Jakie oddziaływania są pomiędzy Eu2+

In this contribution we investigate nontrivial magnetic compound \EZP. The grown from Sn flux single crystals were investigated using both bulk and microscopic techniques, i.e., ac susceptibility, dc magnetization, magnetoresistivity, and M\"ossbauer spectroscopy measurements were performed in wide temperature range (down to \SI{2}{K}).
These measurements were 
enriched
by measurements of magnetization and magnetoresistivity under high pressure (up to \SI{18.7}{GPa}), and theoretical ab initio calculations.
This approach enabled to look into the possible ground state of \EZP{} (including its magnetic structure) and the type of interactions among the magnetic moments of \Euion. 
As a result we propose that in \EZP there is a strong ferromagnetic Eu-Eu exchange coupling within the basal plane sheets based on superexchange via phosphorus ions, and a weaker antiferromagnetic interaction among the more remote Eu neighbours along the crystallographic \cax.
